Yo'LLaVA: Your Personalized Language and Vision Assistant

Large Multimodal Models (LMMs) have shown remarkable capabilities across a variety of tasks (e.g., image captioning, visual question answering). While broad, their knowledge remains generic (e.g., recognizing a dog), and they are unable to handle personalized subjects (e.g., recognizing a user's pet dog). Human reasoning, in contrast, typically operates within the context of specific subjects in our surroundings. For example, one might ask, "What should I buy for my dog's birthday?"; as opposed to a generic inquiry about "What should I buy for a dog's birthday?". Similarly, when looking at a friend's image, the interest lies in seeing their activities (e.g., "my friend is holding a cat"), rather than merely observing generic human actions (e.g., "a man is holding a cat"). In this paper, we introduce the novel task of personalizing LMMs, so that they can have conversations about a specific subject. We propose Yo'LLaVA, which learns to embed a personalized subject into a set of latent tokens given a handful of example images of the subject. Our qualitative and quantitative analyses reveal that Yo'LLaVA can learn the concept more efficiently using fewer tokens and more effectively encode the visual attributes compared to strong prompting baselines (e.g., LLaVA).

==> sections/approach_old.tex <==
% \section{\shortname{}: Making LLaVA to understand specific concept}
\section{\shortname{}: Personalizing LMMs to Understand Specific Concepts}
% \begin{figure}
%     \centering
%     \includegraphics[width=1\textwidth,page=2 ]{figures/framework.pdf}
%     \caption{Framework}
%     % \yh{a minor suggestion: can you change right part to be a positive example? that will be more straightforward } }
%     \label{fig:framework}
% \end{figure}

% Given a handful of images of a subject or person (e.g., 5 images of your plushy) without any textual labels or captions, our goal is to learn about the subject based solely on its visual attributes.
% The ultimate goal is for \shortname{} to recognize the subject in new images during testing (e.g., given a new test image, \shortname{} can recognize that subject in the photo or not) and to support question answering about the subject, regardless of whether images are available (e.g., What is the subject doing in this photo) or without any images (e.g., What is the color of the subject?).

% Given a handful of images of a subject or person (e.g., 5 images of your plush toy) without any textual labels or captions, our goal is to learn about the subject based solely on its visual attributes. The ultimate aim is for \shortname{} to recognize \emph{the subject} in new images during testing (e.g., given a new test image, \shortname{} can recognize whether \emph{the subject} is in the photo or not) and to support question answering about the subject, regardless of whether images are available (e.g., What is \emph{the subject} doing in this photo?) or text-only conversation (without images) (e.g., What is the color of \emph{the subject}?).


Given a handful of images of a subject or person $I_{0}, \dots, I_{n}$ (e.g., 5 images of your plush toy named \texttt{<sks>}) without any textual labels or captions, our goal is to learn about the subject (e.g., identified as \texttt{<sks>}) based solely on its visual attributes. The ultimate aim for \shortname{} is: (1) To recognize \emph{the subject} (\texttt{<sks>}) in new images during testing (e.g., given a new test image, \shortname{} can recognize whether \texttt{<sks>} is in the photo or not); (2) to support visual question answering about the subject (e.g., Given a new photo, ask where is \texttt{<sks>} in this photo?); and (3) to support text-only conversation, or in other words (e.g., one might ask What is the color of \texttt{<sks>}?\yh{without uploading images} ).

% To be specific, given a set of images $I_{0}, \dots, I_{n}$ representing a personalized subject , our goal is to enable \shortname{} to to recognize \emph{the subject} in new images during testing (e.g., given a new test image, \shortname{} can recognize whether \emph{the subject} is in the photo or not) and to support question answering about the subject, regardless of whether images are available (e.g., What is \emph{the subject} doing in this photo?) or text-only conversation (without images) (e.g., What is the color of \emph{the subject}?).

We start by detailing how we represent the subject as a learnable concept for LLaVA~\cite{liu2023llava} in Sec.~\ref{sec:learnable_prompt}. We then delve into the methods used to generate training data in Sec.~\ref{sec:visual-exploration}, followed by a discussion on enhancing understanding through hard negative example enhancement in Sec.~\ref{sec:negative_enhancement}.


\subsection{Personalized subject as learnable prompt}
\label{sec:learnable_prompt}
\begin{wrapfigure}{l}{0.5\textwidth}
    \centering
    \vspace{-0.3cm}
    \includegraphics[width=0.5\textwidth]{figures/training-pipeline.pdf} % Adjust width as needed
    \caption{Training pipeline}
    \label{fig:framework}
    \vspace{-0.3cm}
\end{wrapfigure}
Prompting stands out as the most straightforward and natural way for steer multimodal models. For example, when presented with an image, if one wish to ask whether your personal toy (e.g., called \texttt{<sks>}) is in that image or not, one might begin by providing a personalized description (e.g., ``\texttt{<sks>} is a yellow-white plush shaped like a dog", Table~\ref{tab:prompt_vs_learnable_prompt}, Left).
However, manually crafting such prompts proves cumbersome.
There are also numerous scenarios where an explicit textual prompt fails to precisely or accurately describe the subject (e.g., describing your friend). \yj{It may require a lot of tokens to accurately describe the personalized concept.}
In lieu of manual efforts, we propose to automatically learn this personalized description.
Specifically, when presented with a photo, we aim to learn a sequence of tokens that describe it (Tab~\ref{tab:prompt_vs_learnable_prompt}, Right). This approach is lightweight, requires updating to only a few parameters (new tokens), while leaving core parameters (e.g., language models, image encoder) untouched.
% Furthermore, the length of actual textual prompts is another consideration (e.g., one may need 100-200 words to describe your dogs). On the flip side, much research~\cite{} \lht{CITE} has shown that soft (or sometimes called continuous) \lht{let's see if there're better ways of saying this?} prompts are more effective and efficient for multiple tasks (e.g., summary paragraph like prefix tuning~\cite{}, serving as system prompt~\cite{} for tool calls~\cite{hao2023toolkengpt}).
% \lht{this para looks very similar to the one in the intro.}
% \thao{haha, i agree, i also feel like i read the intro twice}
% Based on these motivations, we define personalization as a learnable soft-prompt.
% Based on these motivations, we define personalization as learning a soft-prompt.

Specifically, given a set of images $I_{0}, \dots, I_{n}$ of a subject, we optimize personalized soft-prompt with $k+1$ trainable tokens $\thetav=$\{\texttt{sks}, \textless\texttt{token}\textsubscript{1}\textgreater, \dots, \textless\texttt{token}\textsubscript{k}\textgreater\} \yh{also classifier's head?} with the personalized prompt: \yj{we need to explain what <sks> is.  is it chosen as a rare token, or added as a new entry in the vocabulary, etc. and why.}
%%%%%% This is non-color verison
% \begin{center}
%     ``\texttt{<sks> is \textless\texttt{token}\textsubscript{1}\textgreater \textless\texttt{token}\textsubscript{2}\textgreater \dots
%     \textless\texttt{token}\textsubscript{k}\textgreater}.''
% \end{center}
% \thao{Choose either color or non-color version}
%%%%%% This is colorful version
\begin{center}
    ``\texttt{\textcolor{orange}{<sks>} is \textcolor{blue}{<$\text{token}_{1}$>}\textcolor{red}{<$\text{token}_{2}$>}$\dots$\textcolor{teal}{<$\text{token}_{k}$>}}.''
\end{center}
For each image $I_{i}$, we generate conversation data  $(\Xmat_{\texttt{q}}^i, \Xmat_{\texttt{a}}^i)$ (detailed in Sec.~\ref{sec:visual-exploration}).
We use the standard masked language modeling loss to compute the probability of the target answers $\Xmat_{\texttt{a}}$ for each conversation of length $L$ by:

\begin{equation}
    p( \Xmat_{\texttt{a}} |  \Xmat_{\texttt{v}}) =
    \prod_{i=1}^{L} p_{\thetav} (  \xv_i
| \Xmat_{\texttt{v}}, \Xmat_{\texttt{a}, <i}),
    \label{eq:auto_regressive}
\end{equation}

where $\thetav$ is the trainable parameters, $L$ is the length of conversation, and $\Xmat_{\texttt{a}, <i}$ are the instruction and answer tokens in all turns before the current prediction token $\xv_i$, respectively. \yj{we need to say explicitly what is not being trained, and also the output layer} \yh{agree, we need more precise. Also please CAREFULLY check notations etc. There are some errors, for example: $ \Xmat_{\texttt{v}}$ is not defined; 'i' is used for both indexing data/images and conversation length}

\subsection{Self-instruction data synthesis}
\label{sec:visual-exploration}

\yh{a MAJOR suggestion: should we swap sec3.2 and sec3.3.? I think it is more natural to first do 'identify' and then 'reasoning'. (that is also how myvlm paper introduce their approach)}


\yh{overall, this sec is a bit hard to understand for the first time reading, maybe swapping sec3.2 and sec3.3 would be easier to understand.}

% To help models learn concepts about objects, we use templates for questions and answers to create a text-based conversation. This is akin to providing soft labels for the visual appearance of the object. An example is given in Tab.~\ref{tab:training_data_example}. \yh{maybe should say something like: in table 2 top part? As this table also includes sec 3.3}  In total, we have 10 template questions. Please refer to Sec.~\ref{sec:appendix_data} for all template questions. All of these questions are basic and intrinsic to the subject (e.g., color, shape). We do not include any complex or high-level understanding questions to avoid incorrect assumptions or potential incorrect responses from LLaVA (e.g., "What is the race of this person?"). \yh{llava seems come out of nowhere. When I first time read here, it is very abrupt; better to first explain that we use LLava to create text based data beforehand.} For each image $I_{i}$, we will ask LLaVA all questions in the template and obtain corresponding answers $(\Xmat_{\texttt{q}}^i, \Xmat_{\texttt{a}}^i)$. However, during training, in order to enforce the trainable tokens to remember the visual aspects of the subject, we do not show image $I_{i}$ (text-only dataset).

To facilitate concept learning in models, we generate text-based conversation using predefined templates for questions and answers. This serves as soft labels for the objects' visual characteristics. For clarity, specific examples are presented in the upper part of Tab.~\ref{tab:training_data_example}.
Our template consists of 10 manually written, basic questions related to intrinsic attributes (e.g., ``What is the hair color of this person"), \yh{what if input image is not a person?}which are detailed in Sec.~\ref{sec:appendix_data}.
To avoid inaccuracies or misinterpretations, we deliberately exclude complex or nuanced questions that require a high-level understanding (e.g., ``What is the race of this person?'').
We employ the LLaVA to generate answer for each image $I_{i}$ by posing all template questions and collecting the corresponding answers $(\Xmat_{\texttt{q}}^i, \Xmat_{\texttt{a}}^i)$.
It is important to note that during training, to better enforce the memorization of visual information by the trainable tokens, we do not expose the model to the image $I_{i}$ (using a text-only dataset). Specifically, in the data synthesis process, we input a question and a photo of the subject, collect the answer, but in the final dataset, the image is removed, leaving only the questions and answers as the training data. \thao{explain this}.
\yh{after reading here, i feel more that we should swap 3.2 and 3.3; otherwise till here reviewers think we did not give images during training at all; then they may have some doubts: how to tell visual differences with hard negative images etc}

To enable the model to recognize subjects in given images, we provide a template for positive recognition question answering. This process involves simple queries, such as asking whether a specific subject (referred to as <sks>) is present in the photo. During training, each image is randomly paired with one of these question answering templates. All questions are framed as binary classifications—essentially yes/no questions to determine if <sks> is visible in the photo (Tab.~\ref{tab:training_data_example}).

\begin{table*}[t]\centering
\begin{minipage}{0.95\columnwidth}\vspace{0mm} \centering
\begin{tcolorbox}[colback=verylightgray,boxrule=1.1pt]
    \centering
      \footnotesize
    \begin{tabular}{p{1\columnwidth} c}
    \VarSty{ {\bf Positive Examples} } & \hspace{-3.4cm} \multirow{3}{*}{\includegraphics[width=2cm]{figures/imgs/shiba-yellow.jpg}} \\
    \textit{1 --- Basic visual Exploration Question Answering} & \\
     \quad \quad Question: What type of object is <sks>? (Note: No image) & \\
     \quad \quad Answer: <sks> is a stuffed animal. & \\
    \textit{2 --- Positive recognition task} & \\
    \quad \quad Question: <image> Can you tell me if you recognize <sks> in this photo? & \\
    \quad \quad Answer: Yes, I can confirm that <sks> is indeed in the photo. & \\
    \hrulefill & \\
   % \VarSty{ {\bf Negative Examples} } & \hspace{-3.4cm} \multirow{2}{*}{\includegraphics[width=2cm]{figures/imgs/not-shiba-yellow.jpg}} \\
   \VarSty{ {\bf Negative Examples} } & \hspace{-3.4cm} \multirow{2}{*}{\includegraphics[width=1.8cm]{figures/imgs/176615014.png}} \\
    \textit{3 --- Negative recognition task} & \\
     \quad \quad Question: <image> Can you check if <sks> is in this photo? & \\
     \quad \quad Answer: I have analyzed the image,
        \newline \null\quad\quad\quad\quad\quad and I can confirm that <sks> is not present in the photo. & \\
    \end{tabular}
\end{tcolorbox}
\vspace{-4mm}
\caption{One example to illustrate the visual personalization conversation. \yj{Are these 3 examples, not 1 example?}}
    \label{tab:training_data_example}
\end{minipage}
\vspace{-4mm}
\end{table*}

\subsection{Automated negative discriminate enhancing}
\label{sec:negative_enhancement}

% \thao{Add motivation based on REACT and related works}
\thao{I think we need a consistent title for this. Maybe "Hard negative mining"? Or do you feel current title (Automated negative dscriminative enhancing" is ok... to be, it's a bit overcomplicated somehow.}

While self-instruction visual data craetion can guide the learning of basic visual attributes of the subject, we have empirically observed that this approach lacks sufficient discrimination.
% For example, if sks is a yellow dog-shaped plush, then basically all the yellow stuffed animals are also sks -- Which we do not want, for example, all the Asian women is you.
\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \vspace{-0.3cm}
    \includegraphics[width=0.4\textwidth]{figures/data-creation.pdf} % Adjust width as needed
    \caption{Data creation}
    \label{fig:data_creation}
    \vspace{-6mm}
\end{wrapfigure}
For example, if \texttt{<sks>} is a yellow dog-shaped plush, then the model basically assumes that all the yellow stuffed animals are also \texttt{<sks>} -- such over-generalization is undesirable. \lht{not sure if we still need the asian woman sample, seems pretty clear already} %, for example, all the Asian women is you
% To adress this challenging, we learn from a seriese of work like REACT, etc. in which they retrieve negative example to train the model on.
To address this challenge, we learn from a series of works~\cite{liu2023react} \lht{maybe cite more}, \yh{agree, also i donot think react is that relevant what we are doing somehow} that leverages retrieval to obtain more and better examples to train the model. \thao{hmm but i think we do need to cite some work that do "hard negative mining"/ retrieval negative mining here}

To this end, we propose to retrieval hard negative example.
% \lht{do we want to create this big name?}
This mechanism aims to improve the model's ability to differentiate between visually similar but conceptually distinct objects. Specifically, during training, we introduce additional negative examples that are visually similar to the target object (e.g., visually similar stuffed animals like \texttt{<sks>}). By exposing the model to a diverse range of visually similar yet conceptually different objects, we encourage it to learn more discriminative features and prevent over-generalization. The negative example will be retrieve from LAION~\cite{schuhmann2022laion} database based on visual similarity search. For each image in the training dataset $I_{i}$, we retrieve top 10 similar images to that images to finally form $n*10$ negative examples for the subject \texttt{<sks>}.  \yj{we need to explain which features and what metric is used for similarity}


